uDistil-Whisper: Label-Free Data Filtering for Knowledge Distillation in Low-Data Regimes

Recent work on distilling Whisper's knowledge into small models using pseudo-labels shows promising performance while reducing the size by up to 50%. This results in small, efficient, and dedicated models. However, a critical step of distillation using pseudo-labels involves filtering high-quality predictions and using only those during training. This step requires ground truth labels to compare with and filter low-quality examples, making the process dependent on human labels. Additionally, the distillation process requires a large amount of data thereby limiting its applicability in low-resource settings. To address this, we propose a distillation framework that does not require any labeled data. Through experimentation, we show that our best-distilled models outperform the teacher model by 5-7 WER points and are on par with or outperform similar supervised data filtering setups. When scaling the data, our models significantly outperform all zero-shot and supervised models. Our models are also 25-50% more compute- and memory-efficient while maintaining performance equal to or better than that of the teacher model. For more details about our models, dataset, and other resources, please visit our GitHub page: https://github.com/UBC-NLP/uDistilWhisper.

==> sections/6_discussion.tex <==
\section{Discussion}\label{sec:discussion}
% or error analysis


==> sections/9_ethics.tex <==
\section{Ethics Statement}\label{sec:ethics}

\textbf{Data Collection and Release.} Given that we collect our data from TV series available on YouTube, we ensure that our use of this data aligns with the principles of fair use, given its application to a non-commercial academic setting. Each annotator of the data was made fully aware of the research objectives of the study and the intended use of their annotations.

% \textcolor{red}{AbdulWaheed2Karima: Can you please write this for our in-house data?}
\noindent\textbf{Intended Use.} We believe our work will embolden further research on distilling small and efficient models from large and powerful foundation models especially applied to medium and low-resource languages. Our results show that small distilled models can yield on-par performance on even better results compared to large teacher models. Therefore, our work can raise the interest among the researchers who work on developing efficient machine learning systems under low resource settings however crucial to a wide range of population.
\\
\noindent \textbf{Potential Misuse and Bias.}
Our distilled models can efficiently generate high-quality transcripts for multiple Arabic dialects and have the potential to be misused. Since there exists little-to-no clarity on the nature of the training data of the teacher model, our distilled models can produce potentially harmful and biased content that they can inherit from the teacher model. In addition to that, in our human evaluation, we find that these are susceptible to generating examples from the training data which raises the threat of information leakage. Therefore, we recommend against our distilled models being used without a careful prior consideration of potential misuse and bias.

==> tables/results-sada.tex <==
\begin{table}[]
\begin{tabular}{cll}
\multicolumn{1}{l}{Dialect} & Test & Valid \\
Najdi                       & 0.0  & 0.0   \\
MTOS                        & 0.0  & 0.0   \\
Khaliji                     & 0.0  & 0.0   \\
Hijazi                      & 0.0  & 0.0   \\
Unknown                     & 0.0  & 0.0  
\end{tabular}
\end{table}
